HAMSt3R: Human-Aware Multi-view Stereo 3D Reconstruction

Recovering the 3D geometry of a scene from a sparse set of uncalibrated images is a long-standing problem in computer vision. While recent learning-based approaches such as DUSt3R and MASt3R have demonstrated impressive results by directly predicting dense scene geometry, they are primarily trained on outdoor scenes with static environments and struggle to handle human-centric scenarios. In this work, we introduce HAMSt3R, an extension of MASt3R for joint human and scene 3D reconstruction from sparse, uncalibrated multi-view images. First, we exploit DUNE, a strong image encoder obtained by distilling, among others, the encoders from MASt3R and from a state-of-the-art Human Mesh Recovery (HMR) model, multi-HMR, for a better understanding of scene geometry and human bodies. Our method then incorporates additional network heads to segment people, estimate dense correspondences via DensePose, and predict depth in human-centric environments, enabling a more comprehensive 3D reconstruction. By leveraging the outputs of our different heads, HAMSt3R produces a dense point map enriched with human semantic information in 3D. Unlike existing methods that rely on complex optimization pipelines, our approach is fully feed-forward and efficient, making it suitable for real-world applications. We evaluate our model on EgoHumans and EgoExo4D, two challenging benchmarks con taining diverse human-centric scenarios. Additionally, we validate its generalization to traditional multi-view stereo and multi-view pose regression tasks. Our results demonstrate that our method can reconstruct humans effectively while preserving strong performance in general 3D reconstruction tasks, bridging the gap between human and scene understanding in 3D vision.

==> tables/8_cam.tex <==
\begin{table*}[h]
    \centering
    \caption{Comparison of \\divine and \textbf{ours}}
    \begin{tabular}{lcccccccccc}
        \toprule
        Activity & Large-Scale & Method & TE & s-TE & AE & RRA\_10 & CCA\_10 & s-CCA\_10 & RTA\_10 & s-RTA\_10 \\
        \midrule
        \multirow{2}{*}{Badminton}  
        & \multirow{2}{*}{\ding{51}} & \divine  & 1.438  & 0.073  & 1.930  & 1.000  & 0.001  & 0.996  & 0.997  & 0.997 \\
        &  & \textbf{\textbf{ours}}    & 2.425  & 0.261  & 6.179  & 0.803  & 0.000  & 0.905  & 0.927  & 0.927 \\
        \cline{3-11}
        \multirow{2}{*}{Basketball}  
        & \multirow{2}{*}{\xmark} & \divine  & 1.591  & 0.113  & 1.584  & 1.000  & 0.112  & 1.000  & 1.000  & 1.000 \\
        &  & \textbf{ours}    & 0.828  & 0.098  & 1.591  & 1.000  & 0.625  & 1.000  & 1.000  & 1.000 \\
        \cline{3-11}
        \multirow{2}{*}{Fencing}  
        & \multirow{2}{*}{\xmark} & \divine  & 2.451  & 0.045  & 1.320  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        &  & \textbf{ours}    & 1.217  & 0.105  & 1.406  & 0.995  & 0.000  & 0.988  & 0.983  & 0.983 \\
        \cline{3-11}
        \multirow{2}{*}{Legoassemble}  
        & \multirow{2}{*}{\xmark} & \divine  & 2.204  & 0.059  & 0.911  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        &  & \textbf{ours}    & 1.714  & 0.049  & 0.713  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        \cline{3-11}
        \multirow{2}{*}{Tagging}  
        & \multirow{2}{*}{\xmark} & \divine  & 3.164  & 0.062  & 2.483  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        &  & \textbf{ours}    & 1.672  & 0.056  & 2.153  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        \cline{3-11}
        \multirow{2}{*}{Tennis}  
        & \multirow{2}{*}{\ding{51}} & \divine  & 0.242  & 0.067  & 2.946  & 1.000  & 0.971  & 1.000  & 1.000  & 1.000 \\
        &  & \textbf{ours}    & 3.739  & 0.055  & 2.589  & 1.000  & 0.000  & 1.000  & 1.000  & 1.000 \\
        \cline{3-11}
        \multirow{2}{*}{Volleyball}  
        & \multirow{2}{*}{\ding{51}} & \divine  & 1.147  & 0.153  & 3.972  & 1.000  & 0.000  & 1.000  & 0.994  & 0.994 \\
        &  & \textbf{ours}    & 1.840  & 0.484  & 7.770  & 0.649  & 0.012  & 0.833  & 0.811  & 0.811 \\
        \midrule
        \multirow{2}{*}{Average}  
        & \multirow{2}{*}{\ding{51}} & \divine  & \textbf{0.942}  & \textbf{0.098}  & \textbf{2.949}  & \textbf{1.000}  & \textbf{0.324}  & \textbf{0.999}  & \textbf{0.997}  & \textbf{0.997} \\
        &  & \textbf{ours}    & 2.668  & 0.267  & 5.513  & 0.817  & 0.004  & 0.913  & 0.912  & 0.912 \\
        \cline{3-11}
        \multirow{2}{*}{Average}  
        & \multirow{2}{*}{\xmark} & \divine  & 2.353  & \textbf{0.077}  & 1.575  & \textbf{1.000}  & 0.028  & \textbf{1.000}  & \textbf{1.000}  & \textbf{1.000} \\
        &  & \textbf{ours}    & \textbf{1.358}  & \textbf{0.077}  & \textbf{1.466}  & \textbf{1.000}  & \textbf{0.156}  & 0.997  & \textbf{1.000}  & \textbf{1.000} \\
        \bottomrule
    \end{tabular}
\end{table*}
